FdConfig: A Constraint-Based Interactive Product Configurator

We present a constraint-based approach to interactive product configuration. Our configurator tool FdConfig is based on feature models for the representation of the product domain. Such models can be directly mapped into constraint satisfaction problems and dealt with by appropriate constraint solvers. During the interactive configuration process the user generates new constraints as a result of his configuration decisions and even may retract constraints posted earlier. We discuss the configuration process, explain the underlying techniques and show optimizations.

==> choco-csp-4.tex <==
Consider a CSP $P = (X,D,C)$ with
%
the set $X = \{Cost, Color, Band\}$ of variables %
%
and their respective domains %
$D = (D_{Cost},D_{Color},D_{Band})$
with  %
$D_{Color} = \{Red,Gold,Black,Blue\}$, $D_{Cost} = \{0,...,1400\}$, and %
$D_{Band} = \{700,800,1000\}$.

\mbox{$C$ $=$ %
$(Band = 700 \rightarrow Color = Blue)$ $\wedge$ $(Cost = Band + 500)$}
is a conjunction of constraints over the variables from $X$.

Solutions of the CSP $P$ are \eg 
$\varsigma_1$ with 
$\varsigma_1(Cost) = 1200$, 
$\varsigma_1(Color) = Blue$, and
$\varsigma_1(Band) = 700$ which is also denoted by
$\varsigma_1 = \{Cost/1200, Color/Blue, Band/700\}$
%
and 
\mbox{$\varsigma_2 = \{Cost/1300,Color/Red,Band/800\}$.}




==> choco-csp-5.tex <==
The valid domains of the CSP $P$ is 
%
$D_{vd} = (\{1200,1300\},D_{Color},\{700,800\})$.





==> conclusion.tex <==
\section{Conclusion and Future Work}
\label{sect:conclusion}

In this paper we discuss an approach on interactive product
configuration based on constraint techniques, which was implemented in
our configurator tool \fdconfig. We gave an overview of the product
configuration domain, feature models, and constraint programming in
this context and introduced our approach.

\smallskip

In \fdconfig we employ a finite domain constraint solver that enables
us to deal with integer attributes and arithmetic constraints in
extended feature models. These constraints are usually not supported
in traditional approaches (\eg SAT, BDDs) or only in restricted
forms. However, this enhanced expressiveness comes at the cost of
performance penalties. We deal with this by applying a preliminary
domain analysis in order to relief the solver of unnecessary
computation time for establishing consistency.  Furthermore, we use a
\multithreading approach to enhance the user experience. This allows
the user to continue configuring in a limited way, even if the overall
computation has not yet finished.

\smallskip

\emph{Future work} will include the further development of the
\multithreading approach. We plan to incorporate multiple solvers that
might use different computation strategies.  For example, the feature
model element with the current GUI focus could be taken into
account. This focus-based computation strategy could additionally
improve user friendliness: Domain elements, that the user might want
to configure most likely, would become available more quickly for
configuration decisions.

\smallskip

Also a more subtle handling of the non-chronological retraction of
constraints promises improvement but needs further investigation.

\smallskip

In order to improve the overall performance we consider adding
support for compilation-based approaches (\ie BDDs). These could be
integrated with the solver in the form of custom constraints to speed
up the search.  If a pre-compiled version of a feature model is
available, the implementation of these constraints could access the
BDD. Otherwise the regular solution methods would be applied.

\smallskip

Transformation-based optimizations should be investigated, too. 
%
%--
%
E.g. \cite{GeskeJohn:01} use a clustering optimization to reduce the
number of constraint-variables and constraints. Using feature models 
(\cite{GeskeJohn:01} directly use constraints) 
may support or even inherently realize a form of clustering. 

%---

Another optimization is presented in \cite{MazoEtAl:11}.
The authors discuss the improvement of efficiency
when solving CSPs as transformation results due to a reformulation of
particular boolean constraints into arithmetic constraints.  While
this representation is available in our approach too, the examination
of similar optimizations may be worth considering in the future.
%
In the approach of \cite{MazoEtAl:11} the structure of feature models
is not preserved. This holds optimization potential as well, but must be
done sensitive to retain a mapping to the feature model to allow an
interactive configuration process as needed in our approach.


==> featureModels.tex <==
\paragraph{Feature models}

are particularly used in the context of software product line
engineering to support the reuse when building software-intensive
products. However, they are of course applicable to many other product
line domains.
%
They stem from the \emph{feature oriented domain analysis methodology}
(FODA) \cite{KangEtAl:90}.

A feature model describes a product domain by a combination of
features, \ie specific aspects of the product which the user can
configure by instantiation and further constraints.
%
A product line is given by the set of possible combinations of
feature alternatives. 

The semantics of feature models is typically mapped to propositional
logics \cite{JanotaBotterweckEtAl:10} and can accordingly be mapped
onto a restricted class of constraint satisfaction problems (\cf
\Sects{sect:CP}), namely constraints of the Boolean domain.
%
While many approaches in the literature (\eg
\cite{Hadzic2004TechRep,Hadzic2004,Janota08}) only consider
constraints of the Boolean domain (including equality constraints),
Benavides et.al. \cite{BenavidesEtAl:05} discuss the realization of
arithmetic computations and cost optimization in a feature model (by
so-called "extra-functional features") which can be represented by
general constraint problems.



==> interactiveConfiguration.tex <==

An interactive product configurator is a tool which allows the user to
specify a product according to his specific needs based on the common
core of the set of all products of a product line.
%
This process can be done interactively, \ie in a step-wise fashion, thus
gradually shrinking the search space of the configuration problem.

For the sake of applicability and user-friendliness, a configurator
requires a number of properties like backtrack-freeness, completeness,
order-independent retraction of decisions, short response times and
others.  These strongly depend on the method\footnote{For a discussion
of the solutions methods see below.} underlying the configurator
system. Cost optimization and arithmetic constraints are a desired
functionality too, but these are seldom supported or only
provided in a very restricted form.

While \emph{completeness} ensures that no solutions are lost,
\emph{backtrack-freeness} \cite{Hadzic2004TechRep,Subbarayan2005} 
guarantees that the configurator only offers decision
alternatives for which solutions remain. Thus, the user can always
generate a valid solution from the current configuration state and
does not need to unwind a decision (i.e. he does not need to
backtrack).
%
The \name{Calculate Valid Domains (CVD) function}
\cite{Hadzic2004TechRep} of a configurator realizes this latter
property.





==> introduction.tex <==
Product lines for mass customization \cite{TsengJiao2001} allow to
fulfill the needs and requirements of the individual consumer while
keeping the production costs low. %
They enhance extensibility and maintainance by re-using the
common core of the set of all products.

\emph{Product configuration} describes the process of specifying a
product according to user-specific needs %and requirements 
based on the 
description of all possible (valid) products (the search space).
%
When done \emph{interactively}, the user specifies the features of the
product step-by-step according to his requirements, thus, gradually
shrinking the search space of the configuration problem.
%
This interactive configuration process is supported by a software tool,
the \emph{configurator}. 

In this paper, we present an approach on interactive product
configuration based on constraint programming techniques.
%
Building on constraints enables us to equip our interactive product
configurator \fdconfig with functionality and expressiveness exceeding
traditional approaches but at the cost of performance penalty which
must be dealt with in turn.

\smallskip

The paper is structured as follows:
%
In \Sects{sect:IC} we briefly review the area of interactive
configuration methods and discuss related work.
%
\Sect{sect:CP} introduces important notions from the constraint
paradigm as needed for the discussion of our approach.
%
We present the constraint-based interactive product configurator
\fdconfig in \Sects{sect:approach}.  There, we introduce
\fdfeatures, a language for the definition of feature models, it's
transformation into constraint problems, and the configuration process
using \fdconfig.  Furthermore, we discuss optimizations and
improvements by analyses and \multithreading.
%
\Sect{sect:conclusion} draws a conclusion and points out directions of
future research.
 
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: t
%%% End: 


==> sequential.tex <==
\subsection{The Configuration Phase}
\label{sect:Sequential}

%--

The second phase of our approach, \ie the configuration phase, starts
with the initialization of \fdconfig before the user can start with
the interactive configuration process.

%--

\paragraph{Model pre-processing.}	
%
The solver reads the CSP-model and performs a feasibility check
(\eg by finding the first solution).
%  
If successful, the configurator computes the valid domains as initial
\emph{model consequences} that derive from the CSP. 
%
The calculation of these model consequences is performed in the same
way as the user consequences are calculated later on in the
interactive user configuration phase (see below). 
%
However, once the model consequences have been computed, they are
immutable during the interactive configuration as they don't depend on
the user decisions.

The current, global consistent state of the solver is recorded. 
%
To this \name{ground level state} the solver can be reset 
when, after a retraction of user constraints, 
a re-computation of the valid domains becomes necessary.

%--

\paragraph{User configuration.} 
%
The user starts a configuration step by executing a configuration
action. This is either a configuration decision, \ie limiting the
domain of a feature- or attribute variable which manifests as a user
constraint or the retraction of a decision made earlier. In this
case the corresponding user constraint is removed from the constraint
system.
% 
User decisions are posted by \fdconfig to the solver as user
constraints.

Now, the solver is activated to establish global consistency and to
find all solutions of the constraint system. These are evaluated to
derive the valid domains.
%
Since the valid domains define the configuration options available to
the user in the next configuration step, the constraint system always
remains feasible after a user decision.

After the user consequences have been computed, the user interface is
updated accordingly and the user can perform the next configuration
action.  

\smallskip

In the usual modus operandi for FD solvers, a CSP is once
declared and then read by the solver which computes and returns
solutions. %
In contrast, for interactive configuration we need to re-calculate
sets of solutions again and again because a sub-set of the constraints
(the user constraints) keeps changing over time as a result of the
user making configuration decisions. 

As the solver maintains a heavyweight internal representation of the
constraint system and reading the CSP-model as well as establishing
consistency are time consuming, the option of re-creating the solver
for every user decision is inapplicable. Therefore we control the
solver from outside by utilizing its backtracking infrastructure and
reset the solver into the aformentioned ground level state in case a
user decision has been retracted.








==> solutionTechniques.tex <==

\paragraph{Solution techniques}
\label{sect:methods}

applied to the interactive configuration problem have been compared
by Hadzic et.al. \cite{Hadzic2004TechRep,Hadzic2004} and Benavides
et.al. \cite{BenavidesEtAl:2010}.
%
They mainly distinguish approaches based on propositional logic on the
one hand and on constraint programming on the other hand.

\smallskip

When using \emph{propositional logic} based approaches, configuration
problems are restricted to logic connectives and equality constraints
(see \eg \cite{Hadzic2004TechRep,Subbarayan2004}). Arithmetic
expressions are excluded because of the underlying solution methods.
% 
These approaches perform in two steps. First, the feature model is
translated into a propositional formula. In the second step the
formula is solved (satisfiability checking, computation of
solutions) by appropriate solvers, in particular \emph{SAT solvers} (as in
\cite{Janota08}) and \emph{BDD-based solvers} (see \eg
\cite{Hadzic2004,Subbarayan2005}).
% 
BDD-based solvers translate the propositional formula into a compact
representation, the BDD (binary decision diagram). % 
While many operations on BDDs can be implemented efficiently,
the structure of the BDD is crucial as a bad variable ordering may
result in exponential size and, thus, in memory blow up.
Therefore the compilation of the BDD is done in an offline phase, 
so a suitable variable ordering can be found and the BDD's size becomes
reasonably small.

\smallskip

%-- CSP

Feature models can be naturally mapped into \emph{constraint systems},
in particular into CSPs.
% 
There are some approaches
\cite{BenavidesEtAl:05,Subbarayan2004} using this
correspondence to deal with interactive configuration problems.
%
These typically work as follows: The feature model is translated into
a constraint satisfaction problem (CSP, see \Def{def:CSP} below) and
afterwards analysed by a CSP solver.
% 
Using this approach, no pre-compilation is necessary. In general it
is possible to use predicate logic expressions and arithmetic
in the feature definitions, even if this is 
not realized in the above mentioned approaches.

%--

Transformations of feature models into programs of CLP languages
(i.e. Prolog systems with constraints) have been shown recently in
\cite{KaratasEtAl:10,MazoEtAl:11}.
However, beside the transformation target beeing different from ours, these
approaches do not focus on using these methods for interactive configuration.

Since our \fdconfig tool aims primarily at the software engineering community
as the main users of feature models, we decided in favour of
a \Java-implementation, which would make later integration with common
software development infrastructure like \name{Eclipse} more easy.


\smallskip


%-- Vergleich und Argumentation

Benavides et.al. \cite{BenavidesEtAl:2010} elaborately compare the
approaches sketched above, particularly with respect to
\emph{performance} and \emph{expressiveness or supported operations,
\resp}
% 
They point out that CSP-based approaches, in contrast to others, can
allow extra functional features \cite{BenavidesEtAl:05,KangEtAl:90}
and, in addition, arithmetic and optimization.
% 
Furthermore, they state that "the available results suggest" that
constraint-based and propositional logic-based approaches "provide
similar performance", except for the BDD-approach which "seems to be
an exception as it provides much faster execution times", but with the
major drawback of BDDs having worst-case exponential size.

%--


\smallskip

Extended feature models with numerical attributes, arithmetic, and
optimization are denominated as an important challenge in interactive
configuration by Benavides et.al.~\cite{BenavidesEtAl:2010}.
%
Our approach aims at this challenge. The main idea is to follow the
constraint-based approach while using the combination of different
constraint methods and concurrency to deal with the computational
cost. At this, a major challange is to support the user when making and
withdrawing decisions in an interactive process. 



